Ravestate: Distributed Composition of a Causal-Specificity-Guided Interaction Policy

In human-robot interaction policy design, a rule-based method is efficient, explainable, expressive and intuitive. In this paper, we present the Signal-Rule-Slot framework, which refines prior work on rule-based symbol system design and introduces a new, Bayesian notion of interaction rule utility called Causal Pathway Self-information. We offer a rigorous theoretical foundation as well as a rich open-source reference implementation Ravestate, with which we conduct user studies in text-, speech-, and vision-based scenarios. The experiments show robust contextual behaviour of our probabilistically informed rule-based system, paving the way for more effective human-machine interaction.

==> A3_formal.tex <==
\section{Formal Specification}
\label{appendix:formalisation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Building Blocks}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}[Slot]
\begin{leftbar}
Given a collection of slots $\Slots$, any slot $\slot[i] \in \Slots$ is a pair $\langle L_i, v_i \rangle$ containing a synchronisation primitive $L_i$ and a value $v_i$. It supports the operations $\mathsc{Read}(\slot[i]) := v_i$ and $\mathsc{Write}(\slot[i], x) := v_i \leftarrow  x$.
The synchronisation primitive $L_i$ is a mutex which ensures mutually exclusive and temporally consistent access to the slot value by supporting atomic $\mathsc{Lock}(L_i)$ and $\mathsc{Unlock}(L_i)$ operations.
\label{def:slot}
\end{leftbar}
\end{definition}

\begin{definition}[Signal]
\begin{leftbar}
Given a collection of signals $\Signals$, any signal $\signal[i] \in \Signals = \langle \text{sid}_i, \text{age}_i^\text{min} \in \mathbb{R}, \text{age}_i^\text{max} \in \mathbb{R}, \confl{Tail}_i \subset \Signals \rangle$, where $\text{sid}_i$ is a unique signal name, is a template for a specific event, which may be instantiated by \textit{spikes} with an age between $\text{age}_i^\text{min}$ and age $\text{age}_i^\text{max}$. The \confl{Tail} set qualifies matching spikes to be caused by spikes from specific signals.
\label{def:signal}
\end{leftbar}
\end{definition}

We mark symbols as \confl{blue} that are required for inter-rule conflict resolution. Their use is explained in Section \ref{chap:conflicts}.

\begin{definition}[Spike]
\begin{leftbar}
Given a collection of spikes $\Spikes$, any spike $\spike[i] \in \Spikes$ is a four-tuple $\langle \text{sid}_i, \text{age}_i \in \mathbb{R}, \confl{Cause}_i \subset \Spikes , \confl{Consumed}_i \subseteq \Slots \cup \Rules \rangle$ which corresponds to an operational instance of any signal $\signal_k \in S$ where the signal name $\text{sid}_k$ matches the reference $\text{sid}_i$ and $\text{age}_\text{k}^\text{min} \leq \text{age}_i \leq \text{age}_\text{k}^\text{max}$.
The function $\mathsc{Eval}: \mathcal{P}(\Spikes), S \rightarrow \mathbb{B}$ formalizes the matching decision between a signal and a set of spikes:
\[
\begin{array}{l}
\mathsc{Eval}(\Spikes, s_\text{sig}) := \exists \spike[k] \in \Spikes (\\
\quad (\text{id}_k = \text{id}_\text{sig}) \land (\text{age}_\text{sig}^\text{min} \leq \text{age}_k \leq \text{age}_\text{sig}^\text{max}) \land\\
\quad \forall \signal[\text{tail}] \in \confl{Tail}_{\text{sig}}(\textsc{Eval}(\confl{Cause}_k, \signal[\text{tail}])))
\end{array}
\]
Furthermore, spikes support the operation \textsc{Age}, which increments $\text{age}_k$ of a spike $\spike_k$ by one:
\[
\mathsc{Age}(\spike_k) := \text{age}_k \leftarrow \text{age}_k + 1
\]
\vspace{-10pt}
\label{def:spike}
\end{leftbar}
\end{definition}

\begin{definition}[Emit-Operation]
\begin{leftbar}
Operation \[ \mathsc{Emit}(\text{id}, \text{cause} \subseteq \Spikes, \Spikes) := \Spikes \leftarrow \Spikes \cup \{ \langle \text{id}, 0, \text{cause} \rangle \} \] modifies the spike set $\Spikes$ by adding a new spike for a signal with the given id and cause spikes.
\end{leftbar}
\end{definition}

\begin{definition}[Condition]
\begin{leftbar}
The set $\mathsc{Cond}(\Signals)$ is a set of Boolean expressions over signals \Signals:
\[
\mathsc{Cond}(\hat{S}) := \mathsc{Cond}(\hat{\Signals} \bigcup_{\mathclap{\strut(\signal[L], \signal[R]) \in \hat{\Signals}^2}}{\{\signal[L] \land \signal[R], \signal[L] \lor \signal[R]\}})
\]
The definition of the $\mathsc{Eval}$ function for conditions is extended as follows: Let $l, r \in \mathsc{Cond}(\Signals)$:
\begin{itemize}
    \item $\mathsc{Eval}(\Spikes,l \lor r) := \mathsc{Eval}(\Spikes,l)\lor\mathsc{Eval}(\Spikes,r)$
    \item $\mathsc{Eval}(\Spikes, l \land r) :=  \mathsc{Eval}(\Spikes,l)\land\mathsc{Eval}(\Spikes,r)$
\end{itemize}
In order to enable structural observations about conditions, the $\mathsc{Dnf}: \mathsc{Cond}(S) \to \mathcal{P}(S)$ operation is defined, which turns any condition into it's disjunctive normal form as a set of disjunctive sets of conjunctive signals.
\label{def:condition}
\end{leftbar}
\end{definition}

\begin{definition}[Rule]
\begin{leftbar}
Given a collection of rules $\Rules$, any rule $\prodrule[i]$ is a six-tuple 
\begin{align*}
    \langle \Slots^R_i \subset \Slots, \Slots^W_i \subset \Slots, \mathsc{on}_i \in \mathsc{Cond(\Signals)},\\
    f_i : \Slots^R_i, \Slots^W_i \rightarrow \mathsc{Result}, \Signals^\text{emit}_i \subset \Signals \rangle
\end{align*}

A rule can write to a set of slots $\Slots^W_i$, read from a set of slots $\Slots^R_i$, execute its rule function $f_i$ in reaction to the condition $\text{\textsc{on}}_i$, and emit or wipe spikes for a subset of signals $\Signals^\text{emit}_i$. The return value of the rule function lambda must be a value $\mathsc{Result}\in \prodruleretset$.
\label{def:rule}
\end{leftbar}
\end{definition}

For the actions associated with \textsc{Delete} and \textsc{Resign}, see Section~\ref{chap:transduction}. We bridge the missing temporal link between slot value changes $v_i$ of a slot $\slot[i] \in \Slots$ and rule execution through \textit{changed-signals}, for which spikes are generated as soon as a slot's $\mathsc{Write}$ operation is executed. This mechanism allows rules to treat slot value changes as events, on which they may condition their contextual validity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Procedures}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{chap:transduction}

The execution of a \sigslot~System occurs in a rule matching loop, which iteratively fires the applicable production rules given the current spike set. A so-called \textit{activation} encapsulates a single production operation, meaning the “consumption” of spikes to execute a particular rule function:

\begin{definition}[Activation]
\begin{leftbar}
Given a collection of activations $\Activations$, any activation $\activation[i] \in \Activations$ is a tuple $\langle \Spikes^A_i \subset \Spikes, \prodrule[i]^A \in \Rules,  \confl{Clocks}_i \subset (\mathcal{P}(\Spikes) \times \mathbb{N}) \rangle$: It tracks a set of spikes $\Spikes_i^A$, which potentially fulfill the condition of it's rule $\prodrule[i]^A$. The $\text{Clocks}_i$ set is required for inter-rule conflict resolution (see Chap.~\ref{chap:conflicts}). Any activation $\activation[i] \in A$ supports operations to modify it's spike set:
\begin{itemize}
    \item $\mathsc{Acquire}(\Spikes^A_i, \spike[i]) := \Spikes^A_i \leftarrow \Spikes^A_i \cup \{\spike[i]\}$
    \item $\mathsc{Reject}(\Spikes^A_i, \spike[i]) := \Spikes^A_i \leftarrow \Spikes^A_i \setminus \{\spike[i]\}$
\end{itemize}
The function $\confl{\textsc{Res}}: \Activations \to \mathcal{P}(\Rules \times \mathcal{P}(\Slots))$, $\confl{\textsc{Res}}(\activation[i]):=\{\prodrule[i]\} \cup P^W_i$ returns resources which will be consumed by the activation's rule.
\label{def:activation}
\end{leftbar}
\end{definition}

We aggregate a combination of rules \Rules, activations \Activations, signals \Signals, spikes $\Spikes$ and slots $\Slots$ into a \textit{context} structure $C = \langle\Rules,\Signals,\Slots,\Spikes,\Activations\rangle$. Such a context fully describes a single \sigslot~system at any given point in time. Its temporal transition follows the \textsc{Run} routine (see Fig.~\ref{fig:context-run}).\par

The \textsc{Run} routine creates activations during the step \textit{"Enforce Activation Existence Rule"}. For the activation collection $\Activations$, the context guarantees that for every signal in a condition $\signal[i] \in \mathsc{ON}_i$ of a rule $\prodrule[i] \in \Rules$, it holds at least one activation which does \textit{not} yet reference a spike which fulfills said signal. This condition is necessary because there must be an activation for the rule ready to "absorb" the spike whenever a particular rule condition requires a generated spike (see Def.~\ref{def:act-existence}).

%\begin{Figure}
%\centering
%\includegraphics[width=0.7\linewidth]{figs/context.png}\vspace{-2em}
%\captionof{figure}{Context \textsc{Run} routine. Blue boxes are notes which contain a formal expression of the process they are linked to. The routine references a fixed update frequency $f$, which holds an upper limit on the number of times a single activation can be updated per second.}
%\label{fig:context-run}
%\end{Figure}


\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figs/context.png}\vspace{-2em}
\caption{Context \textsc{Run} routine. Blue boxes are notes which contain a formal expression of the process they are linked to. The routine references a fixed update frequency $f$, which holds an upper limit on the number of times a single activation can be updated per second.}
\vspace{-1em}
\label{fig:context-run}
\end{figure}


\begin{definition}[Activation Existence Guarantee]
\begin{leftbar}
For every context $C = \langle\Rules,\Signals,\Slots,\Spikes,\Activations\rangle$:
\[
\begin{array}{l}
\forall_{\prodrule[x] \in \Rules}: \forall_{\signal[y] \in \mathsc{ON}_x}: \exists_{\activation[z] \in \Activations}:\\ \quad\prodrule[z]^A = \prodrule[x] \land \lnot \mathsc{Eval}(\Spikes^A_z, s_y)
\end{array}
\]
\label{def:act-existence}
\end{leftbar}
\end{definition}

Generally, this guarantee initiates activations, which live until they have acquired a sufficient spike set fulfilling their rule’s condition. When one of them has acquired the necessary spikes, it executes its rule function and removes itself from the activation set $\Activations$. We describe the lifecycle in Fig.~\ref{fig:act-update}, which depicts a flow-chart of the activation \textsc{Update} routine referenced in Fig.~\ref{fig:context-run}.

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figs/activation.png}\vspace{-1.5em}
\caption{Activation \textsc{Update} routine. This routine is called iteratively by a context \textsc{Run} routine for each of the context $C$'s activations $a_x \in A$. Decisions and processes that are required for conflict resolution are labeled red.}
\vspace{-1.5em}
\label{fig:act-update}
\end{figure}

The execution of fulfilled activations is a parallelised process which follows the \textit{pre-run-checks} decision. Right at the beginning of the activation execution process stands \textit{"acquire locks"}. This refers to invoking $\textsc{Lock}(L_y)$ for every slot $p_y \in P^W_x$ of the updated activation's rule's write-slot collection $P^W_x$. Note, that slots from the corresponding read-slot collection $P^R_x$ are not locked. Only write-access is guaranteed to be exclusive throughout the rule's run-time. For every locked slot, the opposite $\textsc{Unlock}(L_y)$ operation is executed at the end of the activation execution. Once an activation executes a rule function, the function returns an element of $\prodruleretset$:

\begin{itemize}
    \item \textsc{Delete} removes the rule from any rule set that contains it (useful for rules that should execute a limited number of times).
    % This symbol allows a rule to indicate that it wishes to be removed from any rule set it is contained in. This is primarily useful for rules that should only execute a limited number of times.
    \item \textsc{Resign} indicates a failure such that the state machine can fall back to the \textit{"second-best"} rule during conflict resolution.
    % This symbol indicates that a rule function failed. When conflict resolution comes into play, this allows the state machine to fall back to the \textit{"second-best"} rule.
    %\item \textsc{Emit}: This symbol allows a rule to indicate that a new spike for one of the signals it references (see definition) should be generated. The \textsc{Cause} spike-set of the newly emitted spike instance will include all spikes that were necessary to fulfill at least one of the activation's condition's conjunct clauses. 
    %Note, that another means of emitting spikes from a rule function is through slot \textsc{Write} invocations within the rule function, which trigger corresponding slot-changed signal spikes.
    %\item \textsc{Wipe}: This symbol allows a rule to indicate that all spikes for a signal it represents should be wiped from the context. In combination with \textsc{Emit}, this gives the rule full control over whether a spike that represents a certain event should be present in the state machine, or not. 
\end{itemize}

Note, that Fig.~\ref{fig:act-update} also hints at the way we can employ inter-activation conflict resolution in the \textsc{Update}-routine \textit{Pre-run checks}, \textit{Pre-run ops} and \textit{Post-run ops} (see Chap.~\ref{chap:conflicts}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Receptors}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The previous Section illustrated how write-access to a slot by any rule is exclusive for that rule throughout its run-time. This means, that any rule that runs continuously to observe the agent's environment may continuously write updates to a slot, but no other rule will be able to read these updates until the observer rule exits at the end of the context's lifetime. For example, a rule that polls a camera feed for face recognition might write information about visible faces into a respective \textsc{VisibleInterlocutors} slot.\par

% In order to allow long-running observer rules, the idea of \textit{receptor rules} is introduced. Receptors are condition-free rules that can be activated by imperative invocation at any time from within a rule function. This relieves the calling rule from locking the slots it wants to write to: The write operation is deferred to a rule that locks/unlocks its write-slots separately.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Active Engagement}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\label{chap:active}

Until now, rules only activate in reaction to external input. To enable proactive engagement by the system, the context manages the \textsc{activity} slot in the \textit{Update Core Properties} step of the \textsc{Run} routine (see Fig.~\ref{fig:context-run}).
The slot's value is the number of activations that currently hold spikes and do not have the \textit{changed-signal} $\signal_{AC}$ of the \textsc{activity} slot in the condition $\text{\textsc{on}}_i$ of their rule $\prodrule[i]^a$ (see Def.~\ref{def:activity}). A rule is proactive if it reacts to the \textsc{activity} slot value becoming zero.
\begin{definition}[Activity Slot-Value]
\begin{leftbar}
\[
\mathsc{activity} := |\{ \activation[i] \in A | \Spikes^A_i \neq \emptyset \land \signal_{AC} \notin \text{\textsc{on}}_i)\}|
\]
\label{def:activity}
\vspace{-10pt}
\end{leftbar}
\end{definition}
%\[
%\mathsc{activity} := \forall_{\activation[i] \in A} (\Spikes^A_i = %\emptyset \lor \signal_{AC} \in \text{\textsc{on}}_i)
%\]
% TODO explain why not contain prop\_activity.changed


\label{chap:conflicts}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Conflict Types}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Within the \sigslot~System, several conflicts may arise between rule activations, such as the following types:

\begin{enumerate}[label=\Alph*.,leftmargin=*,topsep=3pt,itemsep=-3pt,partopsep=1ex,parsep=1ex]
    \item \textbf{Redundant rule activation}: Multiple activations may run for the same rule with the same spike set. Spike-rule pairs are identified as a critical resource: \textit{No spike may be used to activate the same rule twice.}
    \item \textbf{Concurrent slot write-access:} Activations for multiple rules might want to use the same spikes to write to the same slots (see Fig.~\ref{fig:gra2}). This is the central inter-rule conflict resolution problem: \textit{No single spike may be used to write to the same output slot twice.}
\end{enumerate}

The spike's \textit{Consumed} set tracks rule (type A) and slot (type B) consumption per spike (see Def.~\ref{def:spike}).  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Backward-Chaining of Conditions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Given a spike $\spike[x]$ which an activation $\activation[y]$ requires for writing a slot $\slot[z]$, the state machine must know whether there are any other activations which need $\spike[x]$ for the same purpose, even indirectly: $\spike[x]$ might \textit{cause} an offspring spike $\spike[q]$ with $\spike[x] \in \text{Cause}_q$, which would be used by another activation $\activation[p]$ to write to the same slot $\slot[z]$. In order to anticipate $\activation[p]$, its condition must be \textit{backward-complete}:

\begin{definition}[Backward Completion]
\begin{leftbar}
Given a set of rules $\Rules$ and a rule $\prodrule[p] \in \Rules$, the condition $\mathsc{on}_p$ of $\prodrule[p]$ is backward-complete if
\[
\begin{array}{l}
\forall \signal[x] \in \mathsc{on}_p: \\
\quad \forall \prodrule[q] \in \{ \prodrule_q' \in \Rules \setminus \{\prodrule[p]\} | \signal[x] \in S^\text{emit}_{q'}\}: \\
\quad\quad \forall c_q \in \mathsc{Dnf}(\mathsc{on}_q): \exists c_p \in \mathsc{Dnf}(\mathsc{on}_p): \\
\quad\quad\quad c_q \subseteq c_p \wedge \\
\quad\quad\quad\quad \exists \signal[y] \in c_p: \text{id}_x = \text{id}_y \wedge c_q \subset \text{Tail}_y
\end{array}
\]
\end{leftbar}
\end{definition}

The state machine must be able to make an informed decision about which activation gets to consume a certain spike-slot pair: As can be seen from the example in Fig.\ref{fig:gra2}, it must \textit{anticipate} all rules that will be competing. Note, that consuming a slot-write for an offspring-spike $\delta_k$ will also consume this slot for its parent spikes $\spike[\text{parent}]\in\text{Cause}_k$, and vice versa. The transitive sharing of resources over spike-offspring graphs is modeled in \textit{Causal Groups} (Chap.~\ref{chap:causalgroup}). This is also illustrated in Fig.~\ref{fig:gra2}: Even though the rule $\prodrule[3]$ is not directly consuming spikes for signal $\signal[1]$ it is still competing with rule $\prodrule[1]$, because $\signal[1]$ spikes are \textit{necessary} for $\signal[2]$ spikes. \par

Less formally, in order to be backward-complete, for each signal in a condition, the condition must include at least one conjunction that also contains the possible \textit{causes} for this signal. Notice the role of the signal's \text{Tail} set: It qualifies matching spikes to be caused by spikes from specific signals (see Def. \ref{def:spike}). Facilitating backward-completeness, any implementation must consider that signals can have circular cause-effect relationships.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Causal Group Operations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{chap:causalgroup}

Each causal group equivalence class $[\spike]$ of a spike $\spike \in \Spikes$ represents a disconnected sub-graph within the spike cause-effect graph where critical resources are shared. Given a set of spikes $\Spikes$, the modulo $\Spikes/G$ denotes its set of causal groups (see Def.~\ref{def:causalgroup}). Sometimes, an emitted spike must not be part of the causal group that caused it to allow loops, such that a rule can reactivate itself, and secondary write operations, such that a spike can cause a write to an already written slot. We define this requirement as \textit{Detached Emission}.

\begin{definition}[Causal Group]
\begin{leftbar}
Let $\Spikes$ be a set of spikes and the function $\mathsc{Branch}: \Spikes \to \mathcal{P}(\Spikes)$ be
\[
\mathsc{Branch}(\spike[x]):=\{\spike[x]\} \bigcup_{\mathclap{\spike[y] \in \text{Cause}_x}} \mathsc{Branch(\spike[y])}
\]
The causal group equivalence relation is $G=$
\[
\{(\spike[x],\spike[y]) \in \Spikes^2| \mathsc{Branch}(\spike[x]) \cap \mathsc{Branch}(\spike[y]) \neq \emptyset\}
\]
\label{def:causalgroup}
\vspace{-10pt}
\end{leftbar}
\end{definition}

We can now specify the \textbf{pre-run checks}, \textbf{pre-run ops} and \textbf{post-run ops} of the activation \textsc{Update} routine (see Fig.~\ref{fig:act-update}). All of these processes work over the fulfilled conjunct clause set, specifically it's most useful member (see Def.~\ref{def:max-util-clause}). Note, that the \textsc{Utility} function corresponds to the rule self-information as defined in Section~\ref{chap:utility}.

\begin{definition}[Maximum  Utility Clause]
\begin{leftbar}
The \textbf{M}ost \textbf{U}seful (fulfilled) conjunct \textbf{C}lause of an activation $\activation[x] \in \Activations$ is given by the the function $\textsc{Muc}*: \Activations \to \mathcal{P}(\Signals)$, which is defined as
\[
\mathsc{Muc*}(\activation_x):=\argmax_{\mathclap{\text{clause} \in \mathsc{Dnf}(\mathsc{On}_x)}}(\mathsc{Util}(\text{clause}))
\]
With restriction to fulfilled clauses:
\[
\mathsc{Muc}(\activation_x):=\argmax_{\mathclap{\strut\text{clause} \in \{c \in \mathsc{Dnf}(\mathsc{On}_x)|\mathsc{Eval}(\Spikes^A_x, c) \}}}(\mathsc{Util}(\text{clause}))
\]
Versions which return the max instead of the argmax are labelled \textsc{Mu*} and \textsc{Mu}, respectively.
\label{def:max-util-clause}
\end{leftbar}
\end{definition}

First, the \textsc{Consent}-function makes both type A and type B conflict resolution decisions in \textbf{pre-run checks} (Def. \ref{def:consent}). If $\activation[i] \in \Activations$ is an activation and $\mathsc{Consent}(\activation[i], \Activations)$ returns True, the activation proceeds to \textit{Pre-run ops}. If $\mathsc{Consent}(\activation[i], \Activations)$ returns False, the activation invokes $\mathsc{Pressure}(\activation[i], \Activations)$ (Def. \ref{def:pressure}) to communicate its eager execution state to other activations.

\begin{definition}[Consent-Function]
\begin{leftbar}
Given activation $\activation[i] \in \Activations$ the function $\mathsc{Consent}: \Activations, \mathcal{P}(\Activations) \to \mathbb{B}$ is defined as
\[
\begin{array}{l}
\mathsc{Consent}(\activation[i], \Activations):=\\
\quad \forall \spike[k] \in \Spikes^A_i(\text{Consumed}_k \cap \mathsc{Res}(\activation[i])=\emptyset) \land\\
\quad \forall \activation[p]\in \{\activation[x] \in \Activations | \Spikes^A_i/G \cap \Spikes^A_p/G \neq \emptyset \} \setminus \{\activation[i]\}: \\ \quad\quad \mathsc{Mu*}(\activation[p]) \leq \mathsc{Mu}(\activation[i])
\end{array}
\]
\vspace{-5pt}
\label{def:consent}
\end{leftbar}
\end{definition}

\begin{definition}[Pressure-Operation]
\begin{leftbar}
Given activation $\activation[i] \in \Activations$, the operation \textsc{Pressure} is
\[
\begin{array}{l}
\mathsc{Pressure}(\activation[i], \Activations):=\\
\quad \algfor \activation[p]\in \{\activation[x] \in \Activations | \Spikes^A_i/G \cap \Spikes^A_p/G \neq \emptyset \} \setminus \{\activation[i]\}:\\
\quad\quad \algif \mathsc{Mu*}(\activation[p]) > \mathsc{Mu}(\activation[i]): \algfor g \in \Spikes^A_p/G:\\
\quad\quad\quad \algif (\{g\}\times\mathbb{N}) \cap \text{Clocks}_p = \emptyset:\\
\quad\quad\quad\quad \text{Clocks}_p \leftarrow \text{Clocks}_p \cup \{\langle g, \mathsc{Timeout} \rangle\}
\end{array}
\]
The \textsc{Timeout} hyper-parameter controls how long a higher-utility activation may block
lesser activations from executing.
\label{def:pressure}
\end{leftbar}
\end{definition}

Once the \textsc{Update} routine executes \textbf{pre-run ops} associated with an activation \activation[i], it invokes the \textsc{Activated}-operation (Def. \ref{def:activated}), and rejects spikes which are not fulfilling the most useful fulfilled clause.

\begin{definition}[Activated-Operation]
\begin{leftbar}
Given activation $\activation[i] \in \Activations$, the operation \textsc{Activated} is
\[
\begin{array}{l}
\mathsc{Activated}(\activation[i]) := \algfor \spike[p] \in \Spikes^A_i:\\
\quad \text{Consumed}_p \leftarrow \text{Consumed}_p \cup \mathsc{Res}(\activation[i])
\end{array}
\]
\label{def:activated}
\vspace{-10pt}
\end{leftbar}
\end{definition}

For \textbf{post-run ops}, given $\mathsc{Result}\in\prodruleretset$, either one of the operations \textsc{Resigned} (Def. \ref{def:resigned}) or \textsc{Consumed} (Def. \ref{def:consumed}) is executed. The former if $\mathsc{Resign} \in \mathsc{Result}$, the latter otherwise.

\begin{definition}[Resigned-Operation]
\begin{leftbar}
Given activation $\activation[i] \in \Activations$, the operation \textsc{Resigned} is
\[
\begin{array}{l}
\mathsc{Resigned}(\activation[i]) := \algfor \spike[p] \in \Spikes^A_i:\\
\quad \text{Consumed}_p \leftarrow \text{Consumed}_p \setminus \mathsc{Res}(\activation[i])
\end{array}
%\vspace{-5pt}
\]
\label{def:resigned}
\end{leftbar}
\end{definition}

\begin{definition}[Consumed-Operation]
\begin{leftbar}
Given an activation $\activation[i] \in \Activations$, the operation \textsc{Consumed} is
\[
\begin{array}{l}
\mathsc{Consumed}(\activation[i]) := \algfor \spike[p] \in \Spikes^A_i, \activation[q] \in \Activations: \\
\quad \algif \mathsc{Res}(\activation[q]) \cap \mathsc{Res}(\activation[i]) \neq \emptyset:\\
\quad\quad \algfor \spike[r] \in (\Spikes^A_i \cap \Spikes^A_q):\\
\quad\quad\quad \mathsc{Reject}(\Spikes^A_q, \spike[r])
\end{array}
\]
\label{def:consumed}
\end{leftbar}
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Activation Self-Elimination}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Since a partially fulfilled high-utility activation can block a fulfilled lower-utility activation from firing, we must ensure that a partially fulfilled activation only references its spikes while its condition is satisfiable.\par
We can enforce this requirement for condition signals that have completion. If no activation can cause the desired effect spike given the already acquired cause spikes, then the acquired cause spikes must be rejected.\par
For condition signals that do not have a completion (\textit{primary signals}), the activation's \textit{Clocks} set controls their rejection time-frame: For a specific causal group $[\spike[x]]$, the \textsc{Pressure} operation (see Def.~\ref{def:pressure}) adds a clock $\langle [\spike[x]], \mathsc{Timeout} \rangle$ with a countdown timeout. The timeout is decremented every time \textsc{Update} passes the \textit{Auto-Elimination} step, and reset every time an activation acquires a new spike. If for a specific clock $\langle [\spike[x]], \text{countdown} \rangle \in \text{Clocks}$ the countdown reaches zero, the activation rejects all spikes which belong to the corresponding pressured causal group $[\spike[x]]$.

